Lagrangian Cobordisms between Enriched Knot Diagrams

In this paper, we present new obstructions to the existence of Lagrangian cobordisms in $\mathbb{R}^4$ that depend only on the enriched knot diagrams of the boundary knots or links, using holomorphic curve techniques. We define enriched knot diagrams for generic smooth links. The existence of Lagrangian cobordisms gives a well-defined transitive relation on equivalence classes of enriched knot diagrams that is a strict partial order when restricted to exact enriched knot diagrams To establish obstructions we study $1$-dimensional moduli spaces of holomorphic disks with corners that have boundary on Lagrangian tangles - an appropriate immersed Lagrangian closely related to embedded Lagrangian cobordisms. We adapt existing techniques to prove compactness and transversality, and compute dimensions of these moduli spaces. We produce obstructions as a consequence of characterizing all boundary points of such moduli spaces. We use these obstructions to recover and extend results about ``growing" and ``shrinking" Lagrangian slices. We hope that this investigation will open up new directions in studying Lagrangian surfaces in $\mathbb{R}^4$.

==> references.tex <==
@article {HT2,
    AUTHOR = {Hutchings, Michael and Taubes, Clifford Henry},
     TITLE = {Gluing pseudoholomorphic curves along branched covered
              cylinders. {II}},
   JOURNAL = {J. Symplectic Geom.},
  FJOURNAL = {The Journal of Symplectic Geometry},
    VOLUME = {7},
      YEAR = {2009},
    NUMBER = {1},
     PAGES = {29--133},
      ISSN = {1527-5256},
   MRCLASS = {53D45 (53D40 53D42)},
  MRNUMBER = {2491716},
MRREVIEWER = {Michael J. Usher},
       URL = {http://projecteuclid.org/euclid.jsg/1238592310},
}

@article {ELST,
    AUTHOR = {Eiseman, Phil and Lima, Jonathan D. and Sabloff, Joshua M. and
              Traynor, Lisa},
     TITLE = {A partial ordering on slices of planar {L}agrangians},
   JOURNAL = {J. Fixed Point Theory Appl.},
  FJOURNAL = {Journal of Fixed Point Theory and Applications},
    VOLUME = {3},
      YEAR = {2008},
    NUMBER = {2},
     PAGES = {431--447},
      ISSN = {1661-7738},
   MRCLASS = {53D12 (57R90)},
  MRNUMBER = {2434456},
MRREVIEWER = {Hansj\"{o}rg Geiges},
       DOI = {10.1007/s11784-008-0087-0},
       URL = {https://doi.org/10.1007/s11784-008-0087-0},
}

@article{RS,
title = "Asymptotic behaviour of holomorphic strips",
journal = "Annales de l'Institut Henri Poincare (C) Non Linear Analysis",
volume = "18",
number = "5",
pages = "573-612",
year = "2001",
issn = "0294-1449",
doi = "https://doi.org/10.1016/S0294-1449(00)00066-4",
url = "http://www.sciencedirect.com/science/article/pii/S0294144900000664",
author = "Joel W. Robbin and Dietmar A. Salamon",
abstract = "The asymptotic behaviour of a finite energy pseudoholomorphic strip with Lagrangian boundary conditions in a symplectic manifold is determined by an eigenfunction of the linearized operator at the (transverse) intersection.
RÃ©sumÃ©
Le comportement asymptotique d'une bande pseudoholomorphe d'Ã©nergie finie, Ã  frontiÃšre dans une sous-variÃ©tÃ© Lagrangienne d'une variÃ©tÃ© symplectique, est dÃ©terminÃ© par une fonction propre du problÃšme linÃ©arisÃ© le long de l'intersection (transverse)."
}

@misc{RET,
      title={Refined disk potentials for immersed Lagrangian surfaces}, 
      author={ Dimitroglou Rizell, Georgios and Tobias Ekholm and Dmitry Tonkonog},
      year={2020},
      eprint={1806.03722},
      archivePrefix={arXiv},
      primaryClass={math.SG},
      Note={arXiv:1806.03722}
}

@article {HLS,
    AUTHOR = {Hofer, Helmut and Lizan, V\'{e}ronique and Sikorav, Jean-Claude},
     TITLE = {On genericity for holomorphic curves in four-dimensional
              almost-complex manifolds},
   JOURNAL = {J. Geom. Anal.},
  FJOURNAL = {The Journal of Geometric Analysis},
    VOLUME = {7},
      YEAR = {1997},
    NUMBER = {1},
     PAGES = {149--159},
      ISSN = {1050-6926},
   MRCLASS = {32Q65 (32Q60 53D45)},
  MRNUMBER = {1630789},
       DOI = {10.1007/BF02921708},
       URL = {https://doi.org/10.1007/BF02921708},
}

@article {HWZ,
    AUTHOR = {Hofer, H. and Wysocki, K. and Zehnder, E.},
     TITLE = {Applications of polyfold theory {I}: {T}he polyfolds of
              {G}romov-{W}itten theory},
   JOURNAL = {Mem. Amer. Math. Soc.},
  FJOURNAL = {Memoirs of the American Mathematical Society},
    VOLUME = {248},
      YEAR = {2017},
    NUMBER = {1179},
     PAGES = {v+218},
      ISSN = {0065-9266},
      ISBN = {978-1-4704-2203-5; 978-1-4704-4060-2},
   MRCLASS = {53D45 (14N35 57R17)},
  MRNUMBER = {3683060},
MRREVIEWER = {William Liu},
       DOI = {10.1090/memo/1179},
       URL = {https://doi.org/10.1090/memo/1179},
}

@article {gro,
    AUTHOR = {Gromov, Mikhael},
     TITLE = {Pseudo holomorphic curves in symplectic manifolds},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {82},
      YEAR = {1985},
    NUMBER = {2},
     PAGES = {307--347},
      ISSN = {0020-9910},
   MRCLASS = {53C15 (32F25 53C57 57R15)},
  MRNUMBER = {809718},
MRREVIEWER = {Yakov Eliashberg},
       DOI = {10.1007/BF01388806},
       URL = {https://doi.org/10.1007/BF01388806},
}

@article {HWZgw,
    AUTHOR = {Hofer, H. and Wysocki, K. and Zehnder, E.},
     TITLE = {Applications of polyfold theory {I}: {T}he polyfolds of
              {G}romov-{W}itten theory},
   JOURNAL = {Mem. Amer. Math. Soc.},
  FJOURNAL = {Memoirs of the American Mathematical Society},
    VOLUME = {248},
      YEAR = {2017},
    NUMBER = {1179},
     PAGES = {v+218},
      ISSN = {0065-9266},
      ISBN = {978-1-4704-2203-5; 978-1-4704-4060-2},
   MRCLASS = {53D45 (14N35 57R17)},
  MRNUMBER = {3683060},
MRREVIEWER = {William Liu},
       DOI = {10.1090/memo/1179},
       URL = {https://doi.org/10.1090/memo/1179},
}

@misc{polyfold,
      title={A Polyfold proof of Gromov's Non-squeezing Theorem}, 
      author={Franziska Beckschulte and Ipsita Datta and Irene Seifert and Anna-Maria Vocke and Katrin Wehrheim},
      year={2020},
      eprint={2010.07248},
      archivePrefix={arXiv},
      primaryClass={math.SG},
      Note={	arXiv:2010.07248}
}

@book {wild,
    AUTHOR = {Scorpan, Alexandru},
     TITLE = {The wild world of 4-manifolds},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2005},
     PAGES = {xx+609},
      ISBN = {0-8218-3749-4},
   MRCLASS = {57N13 (14J80 32Q55 57-02 57R17 57R57)},
  MRNUMBER = {2136212},
MRREVIEWER = {Vyacheslav S. Krushkal},
}

@article {ST,
    AUTHOR = {Sabloff, Joshua M. and Traynor, Lisa},
     TITLE = {Obstructions to the existence and squeezing of {L}agrangian
              cobordisms},
   JOURNAL = {J. Topol. Anal.},
  FJOURNAL = {Journal of Topology and Analysis},
    VOLUME = {2},
      YEAR = {2010},
    NUMBER = {2},
     PAGES = {203--232},
      ISSN = {1793-5253},
   MRCLASS = {53D35 (53D12 57R17 57R57)},
  MRNUMBER = {2652907},
MRREVIEWER = {Tobias Ekholm},
       DOI = {10.1142/S179352531000029X},
       URL = {https://doi.org/10.1142/S179352531000029X},
}

@Inbook{Eliashberg1995,
author="Eliashberg, Yakov",
editor="Hofer, Helmut
and Taubes, Clifford H.
and Weinstein, Alan
and Zehnder, Eduard",
title="Topology of 2-knots in â4 and symplectic geometry",
bookTitle="The Floer Memorial Volume",
year="1995",
publisher="Birkh{\"a}user Basel",
address="Basel",
pages="335--353",
abstract="We show in this paper that there exists a deep relationship between the differential topology of S2-knots in â4 and their symplectic geometry. In particular, we use symplectic tools to define a real-valued topological invariant of a knotted S2 in â4 (see Section 3.4 below). Here are the main results which motivate this definition.",
isbn="978-3-0348-9217-9",
doi="10.1007/978-3-0348-9217-9_15",
url="https://doi.org/10.1007/978-3-0348-9217-9_15"
}

@misc{wendl,
      title={Automatic Transversality and Orbifolds of Punctured Holomorphic Curves in Dimension Four}, 
      author={Chris Wendl},
      year={2009},
      eprint={0802.3842},
      archivePrefix={arXiv},
      primaryClass={math.SG},
      Note={	arXiv:0802.3842}
}

@book {MS_Intro,
    AUTHOR = {McDuff, Dusa and Salamon, Dietmar},
     TITLE = {Introduction to symplectic topology},
    SERIES = {Oxford Mathematical Monographs},
   EDITION = {Second},
 PUBLISHER = {The Clarendon Press, Oxford University Press, New York},
      YEAR = {1998},
     PAGES = {x+486},
      ISBN = {0-19-850451-9},
   MRCLASS = {53D35 (53D40 57R17 57R57 57R58)},
  MRNUMBER = {1698616},
MRREVIEWER = {Hansj\"{o}rg Geiges},
}
		
		@book {fooo,
    AUTHOR = {Fukaya, Kenji and Oh, Yong-Geun and Ohta, Hiroshi and Ono,
              Kaoru},
     TITLE = {Lagrangian intersection {F}loer theory: anomaly and
              obstruction. {P}art {II}},
    SERIES = {AMS/IP Studies in Advanced Mathematics},
    VOLUME = {46},
 PUBLISHER = {American Mathematical Society, Providence, RI; International
              Press, Somerville, MA},
      YEAR = {2009},
     PAGES = {i--xii and 397--805},
      ISBN = {978-0-8218-4837-1},
   MRCLASS = {53D40 (53D12)},
  MRNUMBER = {2548482},
MRREVIEWER = {Michael J. Usher},
       DOI = {10.1090/crmp/049/07},
       URL = {https://doi.org/10.1090/crmp/049/07},
}

@incollection {KL,
    AUTHOR = {Katz, Sheldon and Liu, Chiu-Chu Melissa},
     TITLE = {Enumerative geometry of stable maps with {L}agrangian boundary
              conditions and multiple covers of the disc},
 BOOKTITLE = {The interaction of finite-type and {G}romov-{W}itten
              invariants ({BIRS} 2003)},
    SERIES = {Geom. Topol. Monogr.},
    VOLUME = {8},
     PAGES = {1--47},
 PUBLISHER = {Geom. Topol. Publ., Coventry},
      YEAR = {2006},
   MRCLASS = {53D45 (14N35 32G81)},
  MRNUMBER = {2402818},
       DOI = {10.2140/gtm.2006.8.1},
       URL = {https://doi.org/10.2140/gtm.2006.8.1},
}
		
@article {AJ,
    AUTHOR = {Akaho, Manabu and Joyce, Dominic},
     TITLE = {Immersed {L}agrangian {F}loer theory},
   JOURNAL = {J. Differential Geom.},
  FJOURNAL = {Journal of Differential Geometry},
    VOLUME = {86},
      YEAR = {2010},
    NUMBER = {3},
     PAGES = {381--500},
      ISSN = {0022-040X},
   MRCLASS = {53D40 (53D12 53D37)},
  MRNUMBER = {2785840},
MRREVIEWER = {Timothy Perutz},
       URL = {http://projecteuclid.org/euclid.jdg/1303219427},
}
		

@article {floer_morselag, 
    AUTHOR = {Floer, Andreas},
     TITLE = {Morse theory for {L}agrangian intersections},
   JOURNAL = {J. Differential Geom.},
  FJOURNAL = {Journal of Differential Geometry},
    VOLUME = {28},
      YEAR = {1988},
    NUMBER = {3},
     PAGES = {513--547},
      ISSN = {0022-040X},
   MRCLASS = {58F05 (35J65 58E05)},
  MRNUMBER = {965228},
MRREVIEWER = {Jean-Claude Sikorav},
       URL = {http://projecteuclid.org/euclid.jdg/1214442477},
}

@article {floer_unregularized,
    AUTHOR = {Floer, Andreas},
     TITLE = {The unregularized gradient flow of the symplectic action},
   JOURNAL = {Comm. Pure Appl. Math.},
  FJOURNAL = {Communications on Pure and Applied Mathematics},
    VOLUME = {41},
      YEAR = {1988},
    NUMBER = {6},
     PAGES = {775--813},
      ISSN = {0010-3640},
   MRCLASS = {58F05},
  MRNUMBER = {948771},
MRREVIEWER = {Holger Kantz},
       DOI = {10.1002/cpa.3160410603},
       URL = {https://doi.org/10.1002/cpa.3160410603},
}
	
	@book {hummel,
    AUTHOR = {Hummel, Christoph},
     TITLE = {Gromov's compactness theorem for pseudo-holomorphic curves},
    SERIES = {Progress in Mathematics},
    VOLUME = {151},
 PUBLISHER = {Birkh\"{a}user Verlag, Basel},
      YEAR = {1997},
     PAGES = {viii+131},
      ISBN = {3-7643-5735-5},
   MRCLASS = {58D15 (58D27 58F05)},
  MRNUMBER = {1451624},
MRREVIEWER = {Bernd Siebert},
       DOI = {10.1007/978-3-0348-8952-0},
       URL = {https://doi.org/10.1007/978-3-0348-8952-0},
}

@article{bedford-gaveau,
 ISSN = {00029327, 10806377},
 URL = {http://www.jstor.org/stable/2374301},
 author = {Eric Bedford and Bernard Gaveau},
 journal = {American Journal of Mathematics},
 number = {4},
 pages = {975--1009},
 publisher = {Johns Hopkins University Press},
 title = {Envelopes of Holomorphy of Certain 2-Spheres in C2*},
 volume = {105},
 year = {1983}
}

@book {liu,
    AUTHOR = {Liu, Chiu-Chu Melissa},
     TITLE = {Moduli of {J}-holomorphic curves with {L}agrangian boundary
              conditions},
      NOTE = {Thesis (Ph.D.)--Harvard University},
 PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
      YEAR = {2002},
     PAGES = {151},
      ISBN = {978-0493-65757-8},
   MRCLASS = {Thesis},
  MRNUMBER = {2703393},
       URL =
              {http://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqdiss&rft_dat=xri:pqdiss:3051225},
}
}	


@article{RS,
     author = {Robbin, Joel W. and Salamon, Dietmar A.},
     title = {Asymptotic behaviour of holomorphic strips},
     journal = {Annales de l'I.H.P. Analyse non lin\'eaire},
     pages = {573--612},
     publisher = {Elsevier},
     volume = {18},
     number = {5},
     year = {2001},
     zbl = {0999.53048},
     mrnumber = {1849689},
     language = {en},
     url = {http://www.numdam.org/item/AIHPC_2001__18_5_573_0/}
}

@misc{blackwell2020constructions,
      title={Constructions of Lagrangian cobordisms}, 
      author={Sarah Blackwell and Noémie Legout and Caitlin Leverson and Maÿlis Limouzineau and Ziva Myer and Yu Pan and Samantha Pezzimenti and Lara Simone Suárez and Lisa Traynor},
      year={2020},
      eprint={2101.00031},
      archivePrefix={arXiv},
      primaryClass={math.SG}
}

@book {mcduffsalamon_fat,
    AUTHOR = {McDuff, Dusa and Salamon, Dietmar},
     TITLE = {{$J$}-holomorphic curves and symplectic topology},
    SERIES = {American Mathematical Society Colloquium Publications},
    VOLUME = {52},
   EDITION = {Second},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2012},
     PAGES = {xiv+726},
      ISBN = {978-0-8218-8746-2},
   MRCLASS = {53D45 (32Q65 53D35)},
  MRNUMBER = {2954391},
MRREVIEWER = {Mark Alan Branson},
}

@article {arn1,
    AUTHOR = {Arnol'd, Vladimir I.},
     TITLE = {Lagrange and {L}egendre cobordisms. {II}},
   JOURNAL = {Funktsional. Anal. i Prilozhen.},
  FJOURNAL = {Akademiya Nauk SSSR. Funktsional' ny\u{\i} Analiz i ego
              Prilozheniya},
    VOLUME = {14},
      YEAR = {1980},
    NUMBER = {4},
     PAGES = {8--17, 95},
      ISSN = {0374-1990},
   MRCLASS = {57R90 (58C27 58F05)},
  MRNUMBER = {595724},
MRREVIEWER = {V. Oproiu},
}

@incollection {eliash_cobordisme,
    AUTHOR = {Eliashberg, Yakov},
     TITLE = {Cobordisme des solutions de relations diff\'{e}rentielles},
 BOOKTITLE = {South {R}hone seminar on geometry, {I} ({L}yon, 1983)},
    SERIES = {Travaux en Cours},
     PAGES = {17--31},
 PUBLISHER = {Hermann, Paris},
      YEAR = {1984},
   MRCLASS = {57R75 (58G30)},
  MRNUMBER = {753850},
MRREVIEWER = {V. Oproiu},
}

@article {BC_lagrangiancob1,
    AUTHOR = {Biran, Paul and Cornea, Octav},
     TITLE = {Lagrangian cobordism. {I}},
   JOURNAL = {J. Amer. Math. Soc.},
  FJOURNAL = {Journal of the American Mathematical Society},
    VOLUME = {26},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {295--340},
      ISSN = {0894-0347},
   MRCLASS = {53D12 (53D37 53D40 55N22 57R58)},
  MRNUMBER = {3011416},
MRREVIEWER = {Jelena Kati\'{c}},
       DOI = {10.1090/S0894-0347-2012-00756-5},
       URL = {https://doi.org/10.1090/S0894-0347-2012-00756-5},
}

@article {audin_1,
    AUTHOR = {Audin, Mich\`ele},
     TITLE = {Quelques calculs en cobordisme lagrangien},
   JOURNAL = {Ann. Inst. Fourier (Grenoble)},
  FJOURNAL = {Universit\'{e} de Grenoble. Annales de l'Institut Fourier},
    VOLUME = {35},
      YEAR = {1985},
    NUMBER = {3},
     PAGES = {159--194},
      ISSN = {0373-0956},
   MRCLASS = {57R90 (58C27)},
  MRNUMBER = {810672},
MRREVIEWER = {I. Vaisman},
       URL = {http://www.numdam.org/item?id=AIF_1985__35_3_159_0},
}



@book {audin_2,
    AUTHOR = {Audin, Mich\`ele},
     TITLE = {Cobordismes d'immersions lagrangiennes et legendriennes},
    JOURNAL = {Travaux en Cours [Works in Progress]},
    VOLUME = {20},
 PUBLISHER = {Hermann, Paris},
      YEAR = {1987},
     PAGES = {xvi+203},
      ISBN = {2-7056-6056-9},
   MRCLASS = {58F05 (57R90 58G15)},
  MRNUMBER = {903652},
MRREVIEWER = {Alan Weinstein},
}


@book {barsamian,
    AUTHOR = {Barsamian, Mark Harry},
     TITLE = {Normal subgroups of the symplectomorphism group},
      NOTE = {Thesis (Ph.D.)--State University of New York at Stony Brook},
 PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
      YEAR = {2002},
     PAGES = {83},
      ISBN = {978-0496-36435-0},
   MRCLASS = {Thesis},
  MRNUMBER = {2704589},
       URL =
              {http://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqdiss&rft_dat=xri:pqdiss:3088695},
}	
}

@misc{lin,
      title={Exact Lagrangian caps of Legendrian knots}, 
      author={Francesco Lin},
      year={2013},
      eprint={1309.5101},
      archivePrefix={arXiv},
      primaryClass={math.SG}
}
	
		
@article{Sauvaget2004,
abstract = {Dans ce texte, on définit, pour les immersions lagrangiennes de variétés fermées dans $\{\mathbb \{C\}\}^n$, une notion d’aire symplectique enlacée. Puis on construit, dans le cas $n=2$, un certain nombre de surfaces lagrangiennes enlaçant une aire infinie. Dans le cas des surfaces exactes, elles ont le minimum de points doubles possible permis par la théorie (sauf la sphère), c’est-à-dire moins que prévu par quelques conjectures.},
affiliation = {Université Paris 13, UMR 7539, Av J-B Clément, 93430 Villetaneuse (France)},
author = {Sauvaget, Denis},
journal = {Annales de l’institut Fourier},
keywords = {Lagrangian; double points; link},
language = {fre},
number = {6},
pages = {1997-2020},
publisher = {Association des Annales de l'Institut Fourier},
title = {Curiosités Lagrangiennes en dimension 4},
url = {http://eudml.org/doc/116166},
volume = {54},
year = {2004}
}


	
